Learning Hyperplanes for Multi-Agent Collision Avoidance in Space

A core challenge of multi-robot interactions is collision avoidance among robots with potentially conflicting objectives. We propose a game-theoretic method for collision avoidance based on rotating hyperplane constraints. These constraints ensure collision avoidance by defining separating hyperplanes that rotate around a keep-out zone centered on certain robots. Since it is challenging to select the parameters that define a hyperplane without introducing infeasibilities, we propose to learn them from an expert trajectory i.e., one collected by recording human operators. To do so, we solve for the parameters whose corresponding equilibrium trajectory best matches the expert trajectory. We validate our method by learning hyperplane parameters from noisy expert trajectories and demonstrate the generalizability of the learned parameters to scenarios with more robots and previously unseen initial conditions.

==> 3_Preliminaries.tex <==
\section{Preliminaries}

\fernando{
\begin{itemize}
    \item state
    \item controls
    \item shorthand
\end{itemize}}

Throughout this paper, we denote indexing by player and timestep with superscripts and subscripts, respectively. Furthermore, we will adopt Clohessy-Wilshire linearized satellite dynamics, for which the state and controls are given by: 
We use the following shorthand notation:
\begin{subequations}
    \label{shorthand}
    \begin{align*}
        \vars := 
            \begin{bmatrix}
                \vars_1\\
                \vdots\\
                \vars_\horizon
            \end{bmatrix}
        \;\vars_t := 
            \begin{bmatrix}
                \vars_t^{1} \\
                \vdots \\
                \vars_t^{\nplayers}
            \end{bmatrix} 
        \;\vars^i := 
            \begin{bmatrix}
                \vars^i_{1} \\
                \vdots \\
                \vars^i_{\horizon}
            \end{bmatrix}
        \;\vars^{-i} := 
            \begin{bmatrix}
                \vars^{1} \\
                \vdots\\
                \vars^{i - 1}\\
                \vars^{i + 1}\\
                \vdots\\
                \vars^{N}
            \end{bmatrix}.
    \end{align*}
\end{subequations}


\subsection{Game}
Consider a deterministic, infinite, general-sum, dynamic game denoted by the tuple $\game = (\vars_1,\cost,\conseq, \consineq,\params,[\nplayers], [\horizon])$. It is played over discrete time-steps $\tvar \in [\horizon] := \{1, \hdots, \horizon\}$ with a set players denoted by $i \in [\nplayers] := \{1, \hdots, \nplayers\}$. Each player seeks to solve the optimization problem:
\begin{subequations}
\label{game}
\begin{align}
&\min_{\vars^i,\controls^i} \cost^{i}(\vars,\controls;\params)\\
    &\mathrm{subject~to}~\conseq^i(\vars,\controls;\params) = 0\\
    &\qquad \qquad ~~\consineq^i(\vars,\controls;\params) \geq 0\,    
\end{align}
\end{subequations} 
Where we use the following shorthand notation:
\begin{subequations}
    \label{shorthand}
    \begin{align*}
        \vars := 
            \begin{bmatrix}
                \vars_1\\
                \vdots\\
                \vars_\horizon
            \end{bmatrix}
        \;\vars_t := 
            \begin{bmatrix}
                \vars_t^{1} \\
                \vdots \\
                \vars_t^{\nplayers}
            \end{bmatrix} 
        \;\vars^i := 
            \begin{bmatrix}
                \vars^i_{1} \\
                \vdots \\
                \vars^i_{\horizon}
            \end{bmatrix}
        \;\vars^{-i} := 
            \begin{bmatrix}
                \vars^{1} \\
                \vdots\\
                \vars^{i - 1}\\
                \vars^{i + 1}\\
                \vdots\\
                \vars^{N}
            \end{bmatrix}.
    \end{align*}
\end{subequations}
\fernando{Make reference to parameters} Superscripts index by player, subscripts index by timestep and $\var_\tvar^i \in \mathbb{R}^\nstates$, $\control_\tvar^i \in \mathbb{R}^\ncontrols$ denote states and controls, respectively. 
In this paper, we consider an open-loop information structure where every player $i$ specifies its entire control sequence $\controls^i$ given only the initial state of the game $\vars_1$.

\begin{assumption}[Smoothness] For all players, and at all times, the objectives $\cost^i$ and the constraints $\conseq^i$ and $\consineq^i$ have well-defined second derivatives with respect to all state and control variables.
\end{assumption}




==> old.tex <==
\section{Other}

We're trying to solve the following problem 
\begin{subequations}
\label{inference_problem}
\begin{align*}
&\min_{\vars,\controls,\params} \sum_{k = 0}^{\numobs-1}{\norm{\obs_k - \obsmodel_k}^2}\\
    &\mathrm{subject~to}~ (\vars, \controls) \mathrm{~is~a~NE~of~} \game(\params)
\end{align*}
\end{subequations} 
 Consider the following game 
\begin{subequations}
\label{game}
\begin{align*}
&\min_{\var^i,\control^i} \cost^{i}(\vars,\controls;\params)\\
    &\mathrm{subject~to}~\consineq^i(\vars,\controls;\params) \geq 0\,\\
    &\qquad \qquad ~~ \conseq^i(\vars,\controls;\params) = 0
\end{align*}
\end{subequations} 
where a superscript indicates a player index, and a subscript indicates a time index. If we do the slack variable trick, the game now looks like this:
\begin{subequations}
\label{eqn:game_slack}
\begin{align*}
    &\min_{\var^i,\control^i,\slack^i;\params}~\cost^i(\vars,\controls) - \barrierparam\sum_{j = 1}^m{\log{\slack^{i}(j)}} \\ 
    &\mathrm{subject~to}~\consineq^i(\vars,\controls;\params) - \slack^i = 0\\
    &\qquad \qquad ~~ \conseq^i(\vars,\controls;\params) = 0\\
\end{align*}
\end{subequations}   
And the KKT conditions look like this: 
\begin{subequations}
\label{eqn:kkt_slack}
\begin{align*}
\kkt(\vars,\controls,\slacks,\params) =
\begin{bmatrix}
    \kkt^1\\
    \vdots\\
    \kkt^\numplayers
\end{bmatrix}
= 0
\end{align*}
\end{subequations} 
where 
\begin{subequations}
\label{eqn:kkt_slack}
\begin{align}
\kkt^i(\vars,\controls,\slacks,\params) =
\begin{bmatrix}
    \nabla_{\vars}\mathcal{L}^i\\
    \nabla_{\controls}\mathcal{L}^i\\
    \nabla_{\slacks}\mathcal{L}^i\\
    \consineq^i - s^i\\
    \conseq^i\\
\end{bmatrix}
\end{align}
where 
\end{subequations} 
\begin{equation}
    \mathcal{L}^i = 
 \cost^i - \mu\sum_{j = 1}^m{\log{\slack^{i}(j)}} - \lmineq^{i\top}(\consineq^i - \slack^i) - \lmeq^{i\top}\conseq^i
\end{equation}
and the arguments have been omitted for brevity. Therefore, the original problem becomes the following: 
\begin{subequations}
\label{inference_problem_kkt}
\begin{align}
&\min_{\vars,\controls,\slacks,\params} \sum_{k = 0}^{\numobs-1}{\norm{\obs_k - \obsmodel_k(\vars)}^2}\\
    &\mathrm{subject~to}~ \kkt^i(\vars,\controls,\slacks,\params) =

\end{align}
\end{subequations} 


Yue Yu suggestion for a game to solve: think about a situation in which each player is doing the following: 
\begin{subequations}
\label{problem_obstacle_avoidance}
\begin{align*}
&\min_{\var,\control,\params} \sum_{j = 0}^{N-1}{(\var^{i\top}_k\weightstate\var^i_k + \control^{i\top}_k\weightcontrol\control^i_k)}\\
    &\mathrm{subject~to}~ \var^{i}_{k+1} = A\var^i_{k} + B\var^i_{k}\\
    &\qquad \qquad ~~ \var^i_{N} = A\var^i_{k} + B\var^i_{k}\\
    &\qquad \qquad ~~  \normal_k^{\top}\var_k - \radius \geq 0
\end{align*}
\end{subequations} 
where $\normal_k = [\cos(k \params),\, \sin(k\params)]^{\top}$ is the normal of a hyperplane tangent to a keep-out-zone of radius $\radius$ at time $k$. 

In this case, the parameters dictate how fast the  hyperplane rotates around the circle. 
\begin{figure}[h!]
    \centering
    \includegraphics[width=\linewidth,trim = 10 20 10 0]{Figures/KoZ diagram.jpg}
    \caption{Hello world}
    \label{fig:Rotating hyperplane around obstacle}
\end{figure}
In any case, the algorithm would probably go as follows 
\begin{algorithm}[h!]
\DontPrintSemicolon
\caption{Inverse games using interior-point method}\label{alg:scenario-admm}
{
\small
    \textbf{Input:} Make initial guess for $(\vars,\controls,\slacks,\params)$
    
    \While{$\text{Not converged}$}{
        Use nonlinear root finding algorithm (SQP?) to solve for \cref{inference_problem_kkt}.

        Based on results adjust $\barrierparam$. 
    }
    \textbf{Output:} $(\vars,\controls,\slacks,\params)$ such that $\vars, \controls$ are the state and control trajectories for a game parameterized by $\params$.  
}
\vspace{-0.25em}
\end{algorithm}

\pagebreak
\section{Rotating Hyperplane}

\subsection{Game definition}
Two-player hyperplane obstacle avoidance game where each player is trying to get to their objective while avoiding each other. Avoidance is done via one player which always stays on a hyperplane that rotates around a \ac{koz} that's centered on the opponent.

In the following definitions, superscripts and subscripts denote indexing by players and time, respectively, while the bracketed indexing $[\bullet:\bullet]$ denotes indexing into state elements.

\noindent
\textbf{State}
\begin{subequations}
    \begin{align}
        &\vars = 
            \begin{bmatrix}
                \vars_1\\
                \vdots\\
                \vars_\horizon
            \end{bmatrix} \\
        &\vars_t = 
            \begin{bmatrix}
                \vars_t^{1} \\ \vars_t^{2}
            \end{bmatrix}\\
        &\vars_t^i = 
            \begin{bmatrix}
                x^i_t & y^i_t & v^i_t & \theta^i_t 
            \end{bmatrix}^\top
    \end{align}
\end{subequations}


\noindent
\textbf{Cost}
\begin{equation}
    \cost^i = \norm{\vars_T^i[1:2] - \vars_g^i}_2^2 + \norm{\controls^i}_2^2
\end{equation}
where $\vars_g^i$ is the desired final state for Player $i$. This cost encourages goal-seeking behavior while minimizing control effort.  

\noindent
\textbf{Equality constraints}
\begin{equation}
\conseq^i = 
\begin{bmatrix}
    \conseq^i_1 \\
    \vdots \\ 
    \conseq^i_\nconseq \\
\end{bmatrix} = \mathbf{0}.
\end{equation} 
Unicycle dynamics are encoded into the equality constraints by setting $\nconseq = \horizon - 1$ and $\conseq^i_t = \vars^i_{t+1} - \dynamics^i_t(\vars_t, \controls_t)$, where 
\begin{equation}
    \dynamics_t^i(\vars_t,\controls_t) = \vars^i_t + 
    \begin{bmatrix}
        \Delta T v_t^i \cos(\theta_t^i)\\
        \Delta T v_t^i \sin(\theta_t^i)\\
        \controls_t^i
    \end{bmatrix}.
\end{equation}

\noindent
\textbf{Inequality constraints}
\begin{equation}
    \consineq^i = 
            \begin{bmatrix}
                \consineq_1^i\\
                \vdots\\
                \consineq_\nconsineq^i
            \end{bmatrix} \geq 0\\
\end{equation}
where $\geq$ is evaluated element-wise. A rotating hyperplane avoidance constraint is defined by setting $\nconsineq = \horizon$ and
\begin{subequations}
    \begin{align}
        \consineq_t^i &= \hypernormal_t^\top(\vars^i_t[1:2] - \hyperinter_t) \\
        \hypernormal_t &= 
            \begin{bmatrix}
                \cos(\alpha + \omega (t-1))\\
                \sin(\alpha + \omega (t-1))
            \end{bmatrix}\\
        \hyperinter_t &= \vars^2_t[1:2] + \kozrad \hypernormal_t
    \end{align}
\end{subequations}
where $\hyperoffset$ is the initial orientation of the hyperplane normal $\hypernormal$, $\hyperrate$ is rotation rate of the hyperplane, and $\kozrad$ is the \ac{koz} radius.

\noindent
\textbf{Lagrangian}
\begin{equation}
    \lagrangian^i = \cost^i + \underbrace{[\lmeq^{i\top}_1 \hdots \lmeq^{i\top}_{\horizon-1}]}_{\lmeq^{i\top}}
        \begin{bmatrix}
            \conseq^i_1 \\
            \vdots \\ 
            \conseq^i_{\horizon-1}
        \end{bmatrix}
        + \underbrace{[\lmineq^i_1 \hdots \lmineq^i_{\horizon}]}_{\lmineq^{i\top}}
        \begin{bmatrix}
            \consineq^i_1\\
            \vdots \\ 
            \consineq^i_\horizon
        \end{bmatrix}
\end{equation}
where $\lmeq^{i}_t \in \mathbb{R}^{\nstates}, \lmineq^{i}_t \in \mathbb{R}$

\subsection{\ac{kkt} conditions}
\begin{subequations}
\begin{align}
    \nabla_{\vars}\lagrangian^i = 0\\
    \nabla_{\controls}\lagrangian^i = 0\\
    \conseq^i = 0\\
    \consineq^i \geq 0\\
    \lmineq^i \leq 0\\
    \text{Complementary slackness}
\end{align}
\end{subequations}
\subsubsection{$\nabla_{\vars}\lagrangian^i = 0$}
The gradient of Lagrangian with respect to the states $\vars$ is given by  
\begin{equation}
    \nabla_\vars\lagrangian^i = \nabla_\vars\cost^i + \lmeq^{i\top}\nabla_\vars\conseq^i + \lmineq^{i\top}\nabla_\vars\consineq^i.
\end{equation}
The first term is all zeros except for the last block: 
\begin{subequations}
\begin{align}
    \nabla_\vars \cost^i &= 
    \begin{bmatrix}
        \mathbf{0} & \hdots & \mathbf{0} & \nabla_{\vars_\horizon}\cost^i\\
    \end{bmatrix}\\
    \nabla_{\vars_T} \cost^1 &= 2\norm{\vars_T^1[1:2] - x_g^1}_2 
        \begin{bmatrix}
            \vars_T^1[1:2] & \mathbf{0}          
        \end{bmatrix}\\
    \nabla_{\vars_T} \cost^2 &= 2\norm{\vars_T^2[1:2] - x_g^2}_2 
        \begin{bmatrix}
            \mathbf{0} & \vars_T^2[1:2] & \mathbf{0}
        \end{bmatrix}
\end{align}
\end{subequations}
where $\mathbf{0}$ denotes an appropriately sized zero matrix.

$\conseq^i_t$ only depends on Player $i$'s states and controls, namely, $\vars^i_{t+1}$, $\vars^i_{t}$, and $\controls_t^i$. Therefore, the only non-zero Jacobians are the ones obtained by taking the gradient with respect to Player $i$'s states ($x^i$), and can be combined into a single block matrix
\begin{equation}
    \nabla_{\vars^i}\conseq^i = 
        \begin{bmatrix}
            -\nabla_{\vars_1^i}\dynamics_1^i & I \\
            &\ddots\\
            && -\nabla_{\vars_{\horizon-1}^i}\dynamics_{\horizon-1}^i & I
        \end{bmatrix}\\
\end{equation}
In this particular game, both players have the same dynamics, therefore,
\begin{equation}
\nabla_{x_t^i}\dynamics_t^i = 
        \begin{bmatrix}
            1 & 0 & \Delta T \cos(\theta_t^i) & -\Delta T v_t^i \sin(\theta_t^i)\\
            0 & 1 & \Delta T \sin(\theta_t^i) &  \Delta T v_t^i \sin(\theta_t^i)\\
            0 & 0 & 1 & 0 \\ 
            0 & 0 & 0 & 1 \\
        \end{bmatrix}.
\end{equation}
The gradient of the inequality constraints with respect to the states (for both players) is the diagonal block matrix
\begin{subequations}
    \begin{align}
        \nabla_\vars \consineq^i &= 
            \begin{bmatrix}
                \nabla_{\vars_1}\consineq_1^i\\
                &\ddots\\ 
                && \nabla_{\vars_T}\consineq_T^i
            \end{bmatrix}\\
        \nabla_{\vars_t}\consineq_t^i &= 
            \begin{bmatrix}
                \hypernormal_t^\top & 0 & 0 & -\hypernormal_t^\top & 0 & 0 \\
            \end{bmatrix}
    \end{align}
\end{subequations}
Therefore, $\nabla_\vars\lagrangian^i = \begin{bmatrix}
    \nabla_{\vars_1}\lagrangian^i & \hdots & \nabla_{\vars_\horizon}\lagrangian^i
\end{bmatrix}$
where
\begin{multline}
        \nabla_{\vars_t}\lagrangian^i =  \\
        \begin{cases}
            \begin{bmatrix}
                -\lmeq_1^{i\top}\nabla_{\vars_1^i}\dynamics_1^i & \mathbf{0}
            \end{bmatrix} + 
            \lmineq_1^i\nabla_{\vars_1}\consineq_1^i & t = 1\\
            \vspace{0.5mm}\\
            \begin{bmatrix}
               \lmeq_{t-1}^{i\top} -\lmeq_{t}^{i\top}\nabla_{\vars_{t}^i}\dynamics_{t}^i & \mathbf{0}
            \end{bmatrix} 
            + \lmineq_t^i\nabla_{\vars_t}\consineq_t^i & t = 2:(\horizon-1)\\
            \vspace{0.5mm}\\
            \nabla_{\vars_\horizon}\cost^i+
            \begin{bmatrix}
               \lmeq_{t-1}^{i\top} & \mathbf{0}
            \end{bmatrix} 
            + \lmineq_t^i\nabla_{\vars_t}\consineq_t^i & t = \horizon
        \end{cases}
\end{multline}
In implementation, if we assume the initial condition $\vars_{init}$ is known, the first case is not used, and instead the following constraint is enforced:
\begin{equation}
    \vars_{1} = \vars_{init}.
\end{equation}
This effectively removes $\vars_1$ as a decision variable.

\subsection{$\nabla_{\controls}\lagrangian^i = 0$}
Note that player $i$'s controls only appear in its own dynamic constraints. Therefore, it is only necessary to take the gradient of player $i$'s Lagrangian with respect to its own controls $\controls^i$
\begin{equation}
\begin{split}
    &\nabla_{\controls^i}\lagrangian^i = \\ 
    &= \nabla_{\controls^i}\cost^i + \nabla_{\controls^i}(\lmeq^{i\top}\conseq^i) \\ 
    &= \nabla_{\controls^i}\cost^i + 
    \begin{bmatrix}
         \lmeq_1^{i\top}\nabla_{\controls_1^i}\conseq_1^i & \hdots & \lmeq_{\horizon-1}^{i\top}\nabla_{\controls_{\horizon-1}^i}\conseq_1^i & \mathbf{0}
    \end{bmatrix}
\end{split}
\end{equation}
Where the gradients with respect to the cost and constraints are
\begin{subequations}
\begin{align}
    &\nabla_{\controls^i}\cost^i = 
        \begin{bmatrix}
            \nabla_{\controls_1^i}\cost^i & \hdots & \nabla_{\controls_\horizon^i}\cost^i
        \end{bmatrix}\\
    &\nabla_{\controls_t^i}\cost^i = 2\norm{\controls_t^i}_2\controls_t^{i\top}\\
    &\nabla_{\controls_t^i}\conseq_t^i = 
    -\begin{bmatrix}
        0 & 0 \\
        0 & 0 \\
        1 & 0 \\ 
        0 & 1 
    \end{bmatrix}
\end{align}
\end{subequations}

\section{Old Questions}
\begin{itemize}
    \item The proposed game does not have any coupling between players? Isn't it just an optimal control problem for all players that could be solved independently? 
    \item What about framing this in terms of having every player do this when avoiding other players? At every timestep the keep-out zone is another player and is also moving.  
    \item I've got an implementation of the algorithm that adjusts $\barrierparam$ using the Fiacco-McCormick strategy which decreases $\barrierparam$ by scaling it by a constant that's less than one. Would our novel contribution come from having a better way of scaling this parameter based on the fact that we're solving a game? 
    \item Given how ICRA is a robotics conference, might it be a good idea to have some sort of demo? Perhaps if I do the same extension that Lasse did to online planning, we could put this on a robot deciding how to navigate. 
\end{itemize}

\pagebreak

\section{Inverse Game}
\subsection{Game Definition}

In the following definitions, superscripts and subscripts denote indexing by players and time, respectively.

\begin{subequations}
\label{game}
\begin{align*}
&\min_{\var^i,\control^i} \cost^{i}(\vars,\controls;\params)\\
    &\mathrm{subject~to}~\consineq^i(\vars,\controls;\params) \geq 0\,\\
    &\qquad \qquad ~~ \conseq^i(\vars,\controls;\params) = 0
\end{align*}
\end{subequations} 

\noindent
\textbf{State}
\begin{subequations}
    \begin{align}
        &\vars = 
            \begin{bmatrix}
                \vars_1\\
                \vdots\\
                \vars_\horizon
            \end{bmatrix} \\
        &\vars_t = 
            \begin{bmatrix}
                \vars_t^{1} \\
                \vdots\\
                \vars_t^{N}
            \end{bmatrix}\\
        &\vars_t^i = 
            \begin{bmatrix}
                x^i_t & y^i_t & \dot{x}^i_t & \dot{y}^i_t 
            \end{bmatrix}^\top
    \end{align}
\end{subequations}

\noindent
\textbf{Controls}
\begin{subequations}
    \begin{align}
        &\controls = 
            \begin{bmatrix}
                \controls_1\\
                \vdots\\
                \controls_\horizon
            \end{bmatrix} \\
        &\controls_t = 
            \begin{bmatrix}
                \controls_t^{1} \\
                \vdots\\
                \controls_t^{N}
            \end{bmatrix}\\
        &\controls_t^i = 
            \begin{bmatrix}
                \ddot{x}_t^i & \ddot{y}_t^i
            \end{bmatrix}^\top
    \end{align}
\end{subequations}

\noindent
\textbf{Unknown parameters}
\begin{subequations}
    \begin{align}
        \params^i = \begin{bmatrix}
                        \hyperrate^i\\
                        \hyperoffset^i\\
                        \kozrad^i\\
                        \weightstatescalar^i\\
                        \weightcontrolscalar^i\\
                    \end{bmatrix}
    \end{align}
\end{subequations}
Where $\hyperrate, \hyperoffset, \kozrad$ are the hyperplane parameters (explained in detail in the inequality constraints subsection) and $\weightstatescalar, \weightcontrolscalar$ are cost function weights.

\noindent
\textbf{Cost}
\begin{equation}
    \cost^i = \weightstatescalar^i\norm{[x^i_t \enspace y^i_t]^\top - [x^i_g \enspace y^i_g]^\top}_2^2 + \weightcontrolscalar^i\norm{\controls^i}_2^2
\end{equation}
where $[x^i_g \enspace y^i_g]^\top$ is the desired final state for Player $i$. This cost encourages goal-seeking behavior while minimizing control effort.  

\subsection{Equality Constraints}
\begin{equation}
\conseq^i = 
\begin{bmatrix}
    \conseq^i_1 \\
    \vdots \\ 
    \conseq^i_\nconseq \\
\end{bmatrix} = \mathbf{0}.
\end{equation} 
Double integrator dynamics are encoded into the equality constraints by setting $\nconseq = \horizon - 1$ and $\conseq^i_t = \vars^i_{t+1} - \dynamics^i_t(\vars^i_t, \controls^i_t)$, where 
\begin{equation}
    \dynamics_t^i(\vars_t,\controls_t) = \vars^i_t + 
    \begin{bmatrix}
        \Delta T \dot{x}_t^i\\
        \Delta T \dot{y}_t^i\\
        \Delta T \controls_t^i
    \end{bmatrix}.
\end{equation}
\subsection{Inequality Constraints}
\begin{equation}
    \consineq^i = 
            \begin{bmatrix}
                \consineq_1^{i,j}\\
                \vdots\\
                \consineq_\nconsineq^{i,j}\\
                \vdots\\
                \consineq_1^{i,k}\\
                \vdots\\
                \consineq_\nconsineq^{i,k}\\
            \end{bmatrix} \geq 0\\
\end{equation}
where $\geq$ is evaluated element-wise and $\consineq^{i,j}_t$ refers to a constraint shared between players $i$ and $j$ at time $t$. A rotating hyperplane avoidance constraint on player $i$ where the hyperplane is centered on player $j$ is defined by setting $\nconsineq = \horizon$ and
\begin{subequations}
    \begin{align}
        \consineq_t^i &= \hypernormal_t^\top([x^i_t \enspace y^i_t]^{\top} - \hyperinter_t) \\
        \hypernormal_t &= 
            \begin{bmatrix}
                \cos(\hyperoffset^{i,j}_0 + \hyperoffset^{i,j} + \omega^{i,j} (t-1))\\
                \sin(\hyperoffset^{i,j}_0 + \hyperoffset^{i,j} + \omega^{i,j} (t-1))
            \end{bmatrix}\\
        \hyperinter_t &= [x^j_t \enspace y^j_t] + \kozrad^{i,j} \hypernormal_t
    \end{align}
\end{subequations}
where $\hyperoffset_0$ is a feasible reference orientation of the hyperplane normal  $\hypernormal$, $\hyperrate$ is the rotation rate of the hyperplane about player $j$'s position, and $\kozrad$ is the \ac{koz} radius.

\subsection{Inverse Game}
\begin{subequations}
\label{inference_problem_kkt}
\begin{align}
&\min_{\vars,\controls,\slacks,\params}\norm{\obs - \obsmodel(\vars)}_2^2 + \norm{\elastics}_2^2 + \norm{\hyperrate}_2^2 + \norm{\hyperoffset}_2^2 + \norm{\kozrad}_2^2\\
    &\mathrm{subject~to}~\\
    &\quad \quad \quad \quad \begin{bmatrix}
                                \nabla_{\vars}\mathcal{L}^1\\
                                \nabla_{\controls}\mathcal{L}^1\\
                                \nabla_{\slacks}\mathcal{L}^1\\
                                \conseq^1\\
                                \vdots\\
                                \nabla_{\vars}\mathcal{L}^\numplayers\\
                                \nabla_{\controls}\mathcal{L}^\numplayers\\
                                \nabla_{\slacks}\mathcal{L}^\numplayers\\
                                \conseq^\numplayers\\
                              \end{bmatrix} = 0\\
    &\quad \quad \quad \quad \begin{bmatrix}
                                \consineq^1 - s^1\\
                                \vdots\\
                                \consineq^N - s^\numplayers\\
                             \end{bmatrix} = \elastics\\
    &\quad \quad \quad \quad \weightstatescalar^i + \weightcontrolscalar^i = 1 \quad \forall i \in [\numplayers]
\end{align}
\end{subequations} 

\subsection{Inverse game without slacks}
\begin{subequations}
\label{inference_problem_kkt}
\begin{align}
&\min_{\vars,\controls,\params}\norm{\obs - \obsmodel(\vars)}_2^2\\
    &\mathrm{subject~to}~\\
    &\quad \quad \quad \quad \begin{bmatrix}
                                \nabla_{\vars}\mathcal{L}^1\\
                                \nabla_{\controls}\mathcal{L}^1\\
                                \nabla_{\slacks}\mathcal{L}^1\\
                                \conseq^1\\
                                \vdots\\
                                \nabla_{\vars}\mathcal{L}^\numplayers\\
                                \nabla_{\controls}\mathcal{L}^\numplayers\\
                                \nabla_{\slacks}\mathcal{L}^\numplayers\\
                                \conseq^\numplayers\\
                              \end{bmatrix} = 0\\
    &\quad \quad \quad \quad \begin{bmatrix}
                                \consineq^1\\
                                \vdots\\
                                \consineq^N\\
                             \end{bmatrix} \geq 0\\
    &\quad \quad \quad \quad \sum\theta^i = 1 \quad \forall i \in [\numplayers]\\
    & \quad \quad \quad \quad \mathbf{\lambda}\consineq \geq 0
\end{align}
\end{subequations} 
